Report from the NSF Future Directions Workshop on Automatic Evaluation of Dialog: Research Directions and Challenges

This is a report on the NSF Future Directions Workshop on Automatic Evaluation of Dialog. The workshop explored the current state of the art along with its limitations and suggested promising directions for future work in this important and very rapidly changing area of research.

==> human-vs-automatic-evaluation/evaluation-in-practice.tex <==
\subsection{Evaluation Metrics in Practice}

% Assigned: Verena Rieser; Yi-Ting Yeh
%How should we use evaluation metrics in practice? Stand alone, human-in-the-loop evaluation, reinforcement learning, etc.
%- Standardized evaluation metrics should not stay as benchmark that can be overfitted, continue training as there is more data..
%- Human standard is becoming higher and higher so evaluation metrics need to be adjusted to meet the expectation (something flexible and adaptable)
%- Reinforcement learning (unsupervised learning) can be used to point out where the conversation went wrong/well from the overall rating.
%- Given the state-of the technology we may not have a sufficient way of measuring this yet.
%- Reinforcement learning can promote certain aspects (e.g., certain phrases) but may not be good for overall fluency so can be combined with other techniques like s2s model. Before using this, we need a more solid evaluation metric (than BLEU)


%%%%%%%%%%%%%%%%%%%%  YZ/VR draft starts here  %%%%%%%%%%%%%%%%%%%%
%%%%  Minor revisions by JC

While researchers keep developing evaluation metrics which can correlate better with human scores and consider more dialog information, different challenges exist when we want to use those metrics in practice.
First, our current metrics are static, i.e., developed to evaluate capabilities of current systems, but unable to continuously evolve as systems gain greater capabilities. That is, even with the state-of-the-art techniques, the same evaluation metrics might not have a sufficient way of measuring them yet. %if we use standardized evaluation metrics as a benchmark, it has a risk of being poisoned and overfitted.
Therefore, we should consider techniques such as life-long learning or continual learning to improve metrics as more samples are available.


Next, human standards are not static either. People have higher expectations of dialogue systems, and the importance of different dialog aspects might also change.
Therefore, evaluation metrics should be able to adjust accordingly. 
In addition, some aspects of a conversation might be user group specific, e.g.\ dependent on culture or context, and evaluation results might not generalise well beyond that original population.
%The 
Thus, flexibility and adaptability %will be
are two important characteristics for state-of-the-art metrics.


In addition, automatic metrics should be informative to the system developer. 
That is, %besides scores of whole responses or dialogues, it will be beneficial to know exactly where the conversation went wrong or well.
in addition to  scoring entire  responses or entire dialogues, it would be beneficial to know exactly where the conversation went wrong. % or well.
For example, \cite{freitag2021experts} propose a new  evaluation  methodology for Machine Translation grounded  in  explicit  error analysis, based on the Multidimensional Quality  Metrics  (MQM)  framework, which provides insights on type and severity of error. The authors also show that automatic metrics based on word-embeddings have a surprisingly high correlation with MQM scores.


Finally, practical settings might require a trade-off between the  accuracy provided by human evaluation and the cost efficiency of automatic metrics. 
This can be achieved by combining the best of two worlds as proposed in \cite{hashimoto2019unifying}.
The techniques from reinforcement learning or unsupervised learning might be useful to give the information.
However, reinforcement learning might not be good for certain aspects such as overall fluency. 
Exploring how to combine it with other techniques such as Sequence-to-Sequence models will be a promising future direction.

==> human-vs-automatic-evaluation/human-in-evaluation.tex <==
\subsection{Human's Roles in Automatic Evaluation}

% Assigned: Jinho Choi; Samira Shaikh
% Can automatic evaluation convey the human subjectivity inherent in dialog? Different users have different interests? How can we categorize different types of subjectivity? More objective parameters/attributes in evaluation? (e.g., dialog is objectively bad). Separate out objective and subjective aspects of dialog evaluation?
% - Knowledge selection task is subjective, what knowledge can be integrated in dialogue, but difficult to find agreement between subgroups.
% - When teaching a class, even at the same exact school or class, the way you talk needs to be adjusted: the difference between experienced and inexperienced speakers. Majority of others do not know that. It could be difficult to ask machines to do that.
% - Biggest challenge with machines is discrepancy. Certain things are obvious to humans but not to machines, and vice versa.
% - When dealing with dialogue system beyond yes/no, we need to teach basic ability of holding good quality dialogue.
% - Systems should not mislead users.

% Assigned: Milica Gasic; Jinho Choi
% Can automatic metrics replace human evaluation? Or are we only proposing these for automatic metrics?
% - Human evaluation can’t scale. Automatic evaluation can provide more info on more data.
% Need good confidence in the metrics?
% - Since human evaluation is difficult to reproduce → automatic evaluation can be used to maintain consistency
% - Under which criteria can this be done? In some restricted criteria, you could just go with automatic metrics? 
% - Neither human nor automatic evaluation is perfect so we need them both.
% - There are things that machines are better than humans (e.g., knowledge), and the other way so it depends on the metrics and what specific aspects you are looking at.
% - There are so many well-defined NLP benchmarks, but it is a blessing and curse at the same time.

% Assigned: Milica Gasic; Verena Rieser
% Explanations/feedback integrated into the human evaluation? Integrate feedback into metrics
% - Human labor is costly and intense in time


%%%%%%%%%%%%%%%%%%%%  JC draft starts here  %%%%%%%%%%%%%%%%%%%%
\paragraph{Subjectivity.}
What makes dialogue evaluation even more challenging is that subjectivity %, which is generally considered an aspect to be avoided for fair comparison, 
can play a critical role in the evaluation process.
Initiations or responses that are perfectly appropriate for a certain group of people do not necessarily apply to other groups due to sociocultural norms.
Even for the same individual, the way that a dialogue system conducts a conversation may need to change due to the mood or the condition/ context of that individual.
This challenge has been %well-revealed
illustrated by the Alexa Prize Socialbot Grand Challenge where the same bot is evaluated by over a thousand users daily yet the %variant
variation of evaluation scores among those users vary 
%so much because they weight different aspects about the bot.
substantially (cite?). This might be due to different factors, such as individual use of Likert scores, or, in fact, individual preferences.
Similarly, previous work on NLG has observed high disagreement between raters \citep{Walker:2007}, which has been attributed to individual preferences \citep{dethlefs-etal-2014-cluster}

Furthermore, we argue that machine-generated dialogues should not be evaluated in the same way as evaluating translations or paraphrases.
Although all of them can be considered a branch of generation tasks, outputs of translation, paraphrasing, and summarization tasks are more or less a closed set; in other words, it is possible to create a set of gold outputs to evaluate the robustness of models developed for those tasks, whereas it is not the case for the task of (open-domain) dialogue, %management due to this subjectivity,
except for the cases of simple question answering and specific task requests.
Thus, while it is possible to automatically evaluate certain aspects about dialogue that are globally accepted, human evaluation is still necessary to ensure that subjective matters of individuals are still respected in the evaluation.


%%%%%%%%%%%%%%%%%%%%  MG draft starts here   %%%%%%%%%%%%%%%%%%%%
\paragraph{User Testing.}
User testing is a standard and well established procedure in any software development cycle. In terms of dialogue systems research, it is still the most trustful evaluation. A dialogue system is meant to be used by humans so it makes perfect sense to evaluate it with humans. However, this is not without downsides. User evaluation is slow and %very
expensive. It is often very difficult to ensure a wide representation of the user population. In addition, it is difficult to reproduce the results and maintain comparability between evaluations, because each user has their own subjective goal or incentive to use the system. Very rarely the researchers have the ability to have real users evaluate the systems. %Oftentimes these are
Often, evaluations are performed by paid subjects or volunteers, who might not be interested in the actual usefulness of the service. % but rather are curious about “What can it say?”.

Automatic measures on the other hand are cheap, fast, more robust, and therefore scale much better. They also provide easy and simple comparability between different approaches. Many researchers therefore are tempted only to rely on those. The availability of benchmarks in recent years has in this respect been a blessing and a curse. On the one hand, they resulted in many more people building dialogue models, even those who do not have large infrastructure available. This means that many more methods have been proposed and the state-of-the-art has drastically improved. On the other hand, it is less and less likely to find instances where a dialogue model is incorporated in a full dialogue system and evaluated via interaction. Majority of research is evaluated using BLEU or accuracy without any investigation of how that translates to real user experience.

Overall, neither approach in evaluation is bulletproof, which is why we need both. There are aspects of the conversation that are better evaluated by humans and others that are better evaluated by automatic measures.

% MG, my last paragraph above touches this; we could person these paragraphs together
% JC, looks good to me.


%%%%%%%%%%%%%%%%%%%%  MG draft starts here  %%%%%%%%%%%%%%%%%%%%  

With the wide-spread use of supervised learning methods and in particular deep neural network models, %whose performance is measured in terms of accuracy,
it is very easy to loose sight of the fact that dialogue is an interactive task that cannot be fully evaluated using simple corpus-based measures. While human labour is costly and intense, it is important to consider measures which incorporate elements of human evaluation. This has of course to be done with caution. Human feedback can be very noisy, highly subjective and it is not easily generalisable between tasks. Therefore, simply training a predictor of human labels is often not sufficient. However, prior work shows that such an uncertainty-base predictor can to a certain extent be more robust than the human feedback itself~\cite{su-etal-2016-line}. Further research in this direction is necessary.

A related issue is the explainability of a metric. While neural network approaches are to a great extent black box models, there are ways to make them explainable. For example, incorporating attention mechanisms in an automatic neural network-based metric, would mean that the metric could also point what part of the input is desirable or undesirable. One could take a step further and have a natural language feedback generator rather than an overall number as it is known for example that humans are better in giving natural language feedback rather than an objective score that is comparable between different users.


==> human-vs-automatic-evaluation/human-judgement-reliability.tex <==
\subsection{Reliability of human judgements}

% Assigned: Samira Shaikh
% Is correlating to human judgments sufficient?
% - Depends on who the humans are, what the judgements are, and the guidelines given to them. 
% - Identification of hallucination, MTurkers cannot really tell (by looking at short utterances)
% - Human judgements, when/how they are trained, they are often sufficient but not for all situations
% - Human judges have preferences and different ways of evaluation
% - Cognitive biases, coherence scores between machine and human judgements

% Assigned: Dilek Hakkani-Tur; Yizhe Zhang
% Is the human evaluation the gold standard? Subjectivity and first party/third party. How can we make human evaluation reliable/reproducible?
% - Hard to reproduce and consider human evaluation is gold standard
% - Instead of giving out scores to dialogue, compare judgements from multiple systems together.


%%%%%%%%%%%%%%%%%%%%  YZ draft starts here  %%%%%%%%%%%%%%%%%%%%
%%%%  Minor revisions by JC

Human evaluation is thought to be the most reliable signal to assess dialogue systems.
Unfortunately, it has few shortcomings.
First, it is hard to reproduce human evaluation results, and the evaluations from judges can be subjective. 
Second, evaluating conversations in a specific domain may require domain knowledge, which judges might not have.
Third, even with stringent screening of the judges, the quality of the dialogue assessment can still be influenced by multiple factors such as the payment per HIT and the number of annotation cases per judge. 
For instance, the judges may identify quick ``work-around'' solutions to pass the screening without really assessing the dialogue quality (e.g., always prefer the longer response).


%%%%%%%%%%%%%%%%%%%%  VR draft starts here  %%%%%%%%%%%%%%%%%%%%
%%%%  Minor formatting changes by JC
 
Previous research has identified a high degree of inconsistency in human judgements of automatically generated outputs, where ratings often differ significantly ($p<0.001$) for the same utterance \citep{Walker:2007}. %variability
While this might be attributed to individual preference \citep{Walker:2007,dethlefs2014cluster}, \cite{novikova-etal-2018-rankme} also show that consistency (as measured by inter-annotator agreement) can be improved 
by different experimental setup (e.g.\ the use of continuous scales instead of discrete ones).


%%%%%%%%%%%%%%%%%%%%  YZ draft starts here  %%%%%%%%%%%%%%%%%%%%

To make human evaluation more reliable and reproducible, one possible direction is that instead of giving out scores to dialogue, comparing judgements from multiple systems together.
This approach sets up a contrastive assessment to each system, thus can help reduce the subjectivity of the human evaluation process. 

